Piecewise Flat Embedding for Image Segmentation

We introduce a new multi-dimensional nonlinear embedding -- Piecewise Flat Embedding (PFE) -- for image segmentation. Based on the theory of sparse signal recovery, piecewise flat embedding with diverse channels attempts to recover a piecewise constant image representation with sparse region boundaries and sparse cluster value scattering. The resultant piecewise flat embedding exhibits interesting properties such as suppressing slowly varying signals, and offers an image representation with higher region identifiability which is desirable for image segmentation or high-level semantic analysis tasks. We formulate our embedding as a variant of the Laplacian Eigenmap embedding with an $L_{1,p} (0<p\leq1)$ regularization term to promote sparse solutions. First, we devise a two-stage numerical algorithm based on Bregman iterations to compute $L_{1,1}$-regularized piecewise flat embeddings. We further generalize this algorithm through iterative reweighting to solve the general $L_{1,p}$-regularized problem. To demonstrate its efficacy, we integrate PFE into two existing image segmentation frameworks, segmentation based on clustering and hierarchical segmentation based on contour detection. Experiments on four major benchmark datasets, BSDS500, MSRC, Stanford Background Dataset, and PASCAL Context, show that segmentation algorithms incorporating our embedding achieve significantly improved results.

==> pfe-r2.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{sparsity3.pdf}\\
    \includegraphics[width=\columnwidth]{statistic2.pdf}%
    %\includegraphics{statistic2.pdf}
    \vspace{-3mm}
    \caption{Sparsity of edges crossing region boundaries in a locally connected graph. The ratio $r_b$ of boundary length against whole image area in the top-left image is 2.409\%. The $\mathcal{N}_4$-connected graph of a $8\times10$ patch is visualized (top-right). It is divided by a boundary shown in red. Only 9 among 142 edges cross the boundary. Actually the percentage of such edges $r_e$ depends on the length and shape of boundaries. Statical observations in all 2697 groundtruth segmentation maps of BSDS500 are provided in bottom row: approximately linear relation between $r_e$ and $r_b$ (left); distribution of $r_e$ among these segmentation maps (right). Here every pixel is connected to others in a 11$\times$11 neighborhood. Average of $r_b$ and $r_e$ is 2.413\% and 5.113\% respectively. }\vspace{-4mm}  %The bottom-left sub-figure illustrates An statical evidence is shown in
    %percentage of locally connected edges crossing region boundaries.
    %Actually the percentage of such edges $r_e$ in the image is 5.07\% if every pixel is connected to other pixels in a 11$\times$11 neighborhood. }\vspace{-5.3mm}
    \label{fig:sparsity}
\end{figure}

\section{Piecewise Flat Embedding}\label{sec:pfe}
\noindent Let us consider the problem of dividing an image into regions containing pixels with similar low-level/high-level features. We first construct a locally connected graph $G=(V,E)$, where $V$ represents the set of pixels and $E$ represents edges connecting pixels within their neighborhoods. Usually there is only a very small fraction of edges which straddle across region boundaries because of the sparseness of boundaries in 2D image plane -- the majority are between pixels from the same region.
%For the example shown in Figure~\ref{fig:sparsity}, with neighborhood size 11$\times$11, among all the edges in the graph, only a very small fraction (around $5$\%) of them are connections that straddle cross object boundaries -- the majority are between pixels from the same region. %These observations indicate region boundaries might be discovered as the solution to an energy minimization problem with sparsity regularization.
Intuitions and statistical observations in BSDS500 are provided in Figure~\ref{fig:sparsity}. These indicate region boundaries might be discovered as the solution to an energy minimization problem with sparsity regularization.
%This indicates local boundaries are good cues towards the solution to an embedding with sparsity constraint.

Further, we would like to constrain the feature embedding of pixels from the same region to lie as tightly with one another as possible, therefore achieving the goal of piecewise ``flat'' embedding. This piecewise flatness property matters. From one point of view it reduces the intra-class variations of raw pixel values within image segments, for reasons explained earlier. From another point of view, it aims to factorize out a \emph{piecewise smooth} component, which is known as an intrinsic component of pixel values from image formation, and pursues a feature embedding that captures a set of \emph{piecewise constant} representations. This section will describe our formulation of the problem and a numerical solution to it.



%Note that the above observations only hold for locally connected graphs and images where regions are not overly small; otherwise, region boundaries may not comprise a sparse subset of pixels.

%\noindent Let us consider the problem of dividing an image into semantically meaningful regions. We first construct a locally connected graph $G=(V,E)$, where $V$ represents the set of pixels in the image and $E$ represents local connections between every pixel and those pixels inside its neighborhood. For the two images shown in Figure~\ref{fig:sparsity}, if the neighborhood size is 11$\times$11, the percentage of pixels falling on region boundaries is very small (less than $2$\%) because one-dimensional region boundaries typically form a sparse subset of the two-dimensional image plane. Likewise, among all local connections in the graph, the percentage of pairwise connections crossing region boundaries is also very small (around $5$\%) because a majority of connections are formed between pixels from the same region and only a sparse subset of connections straddle sparse boundary pixels. \textcolor{red}{These observations indicate region boundaries might be discovered as the solution to an energy minimization problem with sparsity regularization.??} Note that the above observations only hold for locally connected graphs and images where regions are not overly small; otherwise, region boundaries may not comprise a sparse subset of pixels.


\subsection{Problem Definition} \label{sec:pfedef}
\noindent Given $n$ data points $\mathbf{X} =\{\boldsymbol x_1,\cdot\cdot\cdot, \boldsymbol x_n\}$ in $R^m$, we would like to embed them into a new $d$-demension space $R^d$. Let $\mathbf{Y}=[\mathbf{y}_1,\cdot\cdot\cdot,\textbf{y}_n]^\text{T}$  be the $n$$\times$$d$ data matrix in the new space, where $\mathbf{y}_k^\text{T}$ is the $k$-th row of $\mathbf{Y}$, representing the $d$ coordinates of the $k$-th data point in the new space. %Write $Y_v$ for the $v$-th column of $\mathbf{Y}$, which contains the $v$-th coordinates of all data points.
PFE is to find an embedding $\mathbf{Y}$ that achieves the sparsity, or the piecewise flat property by minimizing the following objective function,
\begin{equation}\label{eq:PFEobj}
    \min_{\mathbf{Y}}\sum_{ij}{\left\|W_{ij}(\mathbf{y}_{i} - \mathbf{y}_{j})\right\|_{1}^{p}} \hspace{5mm} s.t. \hspace{2mm}\mathbf{Y}^{\text T}\mathbf{DY} = \mathbf{I},
\end{equation}
where $0<p\le 1$, $\mathbf{W}=\{W_{ij}\}$ is the symmetric affinity matrix, and $\mathbf{D}$ is the diagonal weight matrix with $D_{ii} = \sum_{j}W_{ji}$. Our embedding formulation is inspired by Normalized Cut and Laplacian Eigenmaps (LE)~\cite{belkin2003laplacian}, which is defined as follows:
\begin{equation}\label{eq:LEobj}
    \min_{\mathbf{Y}}\sum_{ij}{W_{ij}\left\|\mathbf{y}_{i} - \mathbf{y}_{j}\right\|_2^2} \hspace{5mm} s.t. \hspace{2mm}\mathbf{Y}^{\text T}\mathbf{DY} = \mathbf{I},
\end{equation}
where $\mathbf{W}$ and $\mathbf{D}$ are defined in the same way.%, $L = D - W$ is known as the graph Laplacian matrix.


Note $\mathbf{W}$ is a symmetric sparse matrix, %and $W_{ii} = 0$ for $i=1,..,n$. %So we can revise the objective function as follows,\\
%\begin{equation}\label{eq:PFEobjnew}
%    \min_{\mathbf{Y}}\sum_{i}\sum_{j>i}{\left\|W_{ij}(\mathbf{y}_{i} - \mathbf{y}_{j})\right\|_{1}^{p}} \hspace{5mm} s.t. \hspace{2mm}\mathbf{Y}^{T}\mathbf{DY} = \mathbf{I}.
%\end{equation}
so we can rewrite the problem formulation in (\ref{eq:PFEobj}) as follows,
\begin{equation}\label{eq:PFEobjL1p}
    \min_{\mathbf{Y}}{\left\|(\mathbf{M}\mathbf{Y})^{\text{T}}\right\|_{1,p}^{p}} \hspace{5mm} s.t. \hspace{2mm}\mathbf{Y}^{\text T}\mathbf{DY} = \mathbf{I},
\end{equation}
where $\mathbf{M}=\{M_{ij}\}$ is a $t$$\times$$n$ matrix, $M_{ki}=W_{ij}=-M_{kj}$ are for data points $\boldsymbol x_i$ and $\boldsymbol x_j$ that form the $k$-th non-zero entry of the affinity matrix, and $t$ is the total number of non-zero entries. $\left\|\mathbf{A}\right\|_{q,p} = (\sum_{j}(\sum_{i}{|A_{ij}|^q})^{p/q})^{1/p}$ is the $L_{q,p}$ norm of matrix $\mathbf{A}$.

Similarly, the Laplacian Eigenmaps formulation (\ref{eq:LEobj}) can be rewritten as follows,
\begin{equation}\label{eq:LEobjs}
    \min_{\mathbf{Y}}{\left\|(\mathbf{M^\prime}\mathbf{Y})^{\text{T}}\right\|_{2,2}^{2}} \hspace{5mm} s.t. \hspace{2mm}\mathbf{Y}^{\text T}\mathbf{DY} = \mathbf{I},
\end{equation}
where $\mathbf{M^\prime}$ is a $t$$\times$$n$ matrix, $M_{ki}^{\prime}=W_{ij}^{1/2} = -M_{kj}^{\prime}$ are for data points $\boldsymbol x_i$ and $\boldsymbol x_j$ that form the $k$-th non-zero entry of $\mathbf{W}$.

Although (\ref{eq:PFEobjL1p}) and (\ref{eq:LEobjs}) are similar,
the most obvious difference is that we use the $L_{1,p}$ norm in (\ref{eq:PFEobjL1p}) while the formulation of Laplacian Eigenmaps inherits a common trait of mainstream multi-dimensional embedding methods, which is the use of the squared $L_{2,2}$ norm in the objective function.
%This allows the problem to be reduced to an eigendecomposition problem with a closed form solution.
In fact, such a small difference has the following important implication.
The $L_{1,p}$ norm promotes sparse solutions while the $L_{2,2}$ norm does not. A sparse solution implies that, among all locally connected point pairs, there only exists a sparse subset of point pairs whose distances in the new space are sufficiently large, and the distances between the rest of the point pairs are almost zero. Such a sparse solution suggests points with a large distance in the new space should belong to different clusters and points with a very small distance in the new space should belong to the same cluster. Therefore, performing clustering in the new space becomes a straightforward process. On the other hand, although the affinity matrix in (\ref{eq:LEobjs}) attempts to move points with similar attributes closer in the new space, the resulting pairwise distances in the new space still follows a relatively smooth distribution because the measurement of pairwise affinity is coarse and noisy, and the distinction between similar points and dissimilar points is not as clear as in our results.

In the context of image segmentation, a sparse solution to (\ref{eq:PFEobjL1p}) means there only exist a sparse subset of locally connected pixel pairs whose pairwise difference in the new space, $\mathbf{y}_{i}-\mathbf{y}_{j}$, remains sufficiently different from zero. Since the affinity $W_{ij}$ appears together with $\|\mathbf{y}_{i}-\mathbf{y}_{j}\|_1$, a large affinity forces $\|\mathbf{y}_{i}-\mathbf{y}_{j}\|_1$ to approach zero and $\|\mathbf{y}_{i}-\mathbf{y}_{j}\|_1$ becomes nonzero only when the affinity is relatively small. On the other hand, pixel pairs crossing region boundaries typically have smaller affinities than those from the same region. Therefore, the sparse solution to (\ref{eq:PFEobjL1p}) should be capable of facilitating the discovery of region boundaries.
At the interior of a region, $\mathbf{y}_{i}-\mathbf{y}_{j}$ would be most likely zero due to the large affinity between them. This implies each embedding channel has an almost constant value inside every region, hence, the name {\em piecewise flat embedding}.

%\subsection{Justification}  \label{sec:justify}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth,clip,trim=0 0 0 400]{embeddinghists7.pdf}
    \includegraphics[width=\columnwidth,clip,trim=0 412 0 0]{embeddinghists7.pdf}\vspace{-2mm}
    \caption{Laplacian Eigenmaps (top row) and PFE (third row) embedding results, and histograms of each embedding channel. PFE channels are almost piecewise constant while LE channels are piecewise smooth. Because of the adopted $L_{1,p}$ norm, the histograms of our results are much sparser than those of Laplacian Eigenmaps. }\vspace{-4mm}
    \label{fig:embhists}
\end{figure}

%Let $\mathbf \Delta=[\boldsymbol \delta_1,\cdot\cdot\cdot,\boldsymbol \delta_t]^{\text T}$ be a $t\times d$ dimensional matrix, where $\boldsymbol \delta_k=|\mathbf y_i-\mathbf y_j|$ if $\boldsymbol x_i$ and $\boldsymbol x_j$ form the $k$-th pair. According to the above analysis, $\mathbf{\Delta}$ should be a highly sparse matrix under ideal conditions. Referring to the theory of sparse signal recovery \cite{donoho1989uncertainty},\cite{donoho1992signal}, our proposed piecewise flat embedding which uses a $L_{1,p}$-regularized ($0<p\le 1$) objective function as in Eq. (\ref{eq:PFEobjL1p}), should be capable of facilitating the discovery of sparse cluster boundaries.
A visual comparison between our $L_{1,1}$-regularized PFE and Laplacian Eigenmaps are shown in Figure~\ref{fig:embhists}, where each image represents pixelwise values of one embedding channel and the histogram below each image represents the pixel distribution of that embedding channel. According to the results in this figure, PFE channels are almost piecewise constant and their histograms are much sparser than those of Laplacian Eigenmaps, which still possess obvious nonzero gradients within image regions.
%confirms the motivation of designing our method which is to suppress intra-cluster variations while preserving inter-cluster variations. Further verifications on accuracy of our embedding method are in ~\autoref{sec:segmentation} and ~\autoref{sec:clustering}.

\noindent \textbf{Constraint and Total Variation}
%We will discuss the connection between Laplacian eigenproblems with our objective function (\ref{eq:PFEobj}) for $p=1$. Nonlinear eigenproblems are summarized into the following function in~\cite{hein2010inverse},
%\begin{equation}\label{eq:LEp}
%F(y) = R(y)/S(y),
%\end{equation}
%where $R(y)$ and $S(y)$ ($\mathbb R^n \rightarrow \mathbb R_+$) are convex, Lipschitz continuous, even and positively $p$-homogeneous functions with $p\geq 1$. According to the above function, we can define an $L_1$-regularized Laplacian eigenproblem with $L_2$ normalization as follows.
%\begin{definition}\label{def:L11Laplacian}
%Assume $R(y)=\|\mathbf M y\|_1$ and $S(y)=\|\mathbf D^{1/2}y\|_2^2$. $F(y)$ represents an $L_1$-regularized Laplacian eigenproblem. The $u$-th smallest eigenvalue $\lambda_u$ and its corresponding eigenvector $y_u^\ast$ are defined as,
%\begin{align}
%\nonumber y_u^{\ast} &= \argmin_y R(y)&s.t.\;&S(y)=1;\\
%  &  & &  \forall v <u,\; y^{T}\mathbf D y_v^\ast=0.\\
%\lambda_u &= R(y_u^\ast)/S(y_u^\ast).& &
%\end{align}
%\end{definition}The $L_{1,1}$-regularized version of
The constraint in (\ref{eq:PFEobjL1p}) which is inherited from Laplacian Eigenmaps can be decomposed into the following formulations,
\begin{align}
\label{eq:normal} \min_{\mathbf{Y}}{\left\|(\mathbf{M}\mathbf{Y})^{\text{T}}\right\|_{1,p}^{p}} \hspace{4mm} s.t. \; &\forall u,\; y_u^{\text{T}}\mathbf{D}y_u=1;  \\
\label{eq:orthog} &\forall u,\; \forall v\neq u,\;  y_u^{\text T}\mathbf{D}y_v=0 ;
\end{align}
where $y_u$ is the $u$-th column of $\mathbf Y$. The first condition (\ref{eq:normal}) indicates every embedding channel is balanced using a normalized criteria as in~\cite{shi2000normalized}. The second condition (\ref{eq:orthog}) makes different embedding channels orthogonal to each other, which improves the diversity of the embedding channels.

%\begin{theorem}
%The $d$ smallest eigenvalues in Definition \ref{def:L11Laplacian} forms a global optimal solution of (\ref{eq:PFEObjL11s}), $[y_1^*, y_2^*,\cdots,y_d^*]$.
%\end{theorem}
%\noindent Proof is provided in Appendix. Thus our $L_{1,1}$-regularized objective function can be regarded as a general extension of the Laplacian eigenproblem in Definition \ref{def:L11Laplacian}. $p<1$ is not discussed here for its non-convexity.

The discretized total variation regularization~\cite{rudin1992nonlinear} has been frequently used in computer vision tasks such as image smoothing~\cite{min2014fast} and motion estimation~\cite{werlberger2010motion}. A typical image restoration/smoothing objective function with weighted nonlocal total variation regularization~\cite{gilboa2008nonlocal} can be written as follows,
\begin{equation}
\min_{\mathbf{Y}} \| \mathbf{Y}-\mathbf{Y}_0\|_{2,2}^2+\kappa\sum_{ij}W_{ij}\|\mathbf y_i-\mathbf y_j\|_2^2,
\label{eq:WNonlocalTV}
\end{equation}
where $\mathbf Y$ represents the restored/smoothed result and $\mathbf Y_0$ is the input image. $\kappa$ is a constant and $W_{ij}$ is usually computed from a guidance image. The first term in the above formulation is a data term, which uses the input image as a soft constraint to avoid a trivial optimal solution. The above problem can be solved using weighted least squares~\cite{farbman2008edge}. $L_p$-regularized total variation has been used in \cite{min2014fast}. Dynamic guidance is exploited with the help of Welsch's function in~\cite{ham2015robust}. Because of the data term, results from total variation formulations are typically enhanced/restored images whose channels strictly correspond to channels in the input image. Our objective function in (\ref{eq:PFEobj}) utilizes a similar variational regularization with the $L_{1,p}$ norm. However, the data term in total variation formulations is replaced with the orthogonality constraint in our formulation. The adoption of the orthogonality constraint gives us more freedom to define novel embedding spaces that are more independent of the input image. For instance, the dimensionality of an embedding space can be different from that of the input image, and embedding channels do not have to correspond to channels of the input image. Nonetheless, this freedom brings numerical challenges.

%\begin{equation}\label{eq:TVL1pobj}
%    \min_{\mathbf{Y}}{\left\|(\mathbf{M}\mathbf{Y})^{\text{T}}\right\|_{1,p}^{p}} \hspace{5mm} s.t. \hspace{2mm}\mathbf{Y} = \mathbf{Y}_0.
%\end{equation}
%However, the orthogonality constraint used in (\ref{eq:PFEobj}) can be decomposed as follows,
%\begin{equation}\label{eq:orthogconstraint}
%\|\mathbf{D}^{1/2}Y_u\|_2=1,\;Y_u^T\mathbf{D}Y_v=0,\;\forall v\neq u \in\{1,\cdots,d\},
%\end{equation}
%where $Y_u$ is the $u$-th dimension of $\mathbf Y$. The constraint allows the embedding space to be diverse instead of being dependent upon the space of the input data. For example, the embedding space can have a different dimensionality and the embedding channels do not have to approximate the input data.
%\begin{equation}
%\min_{\mathbf{u}} \sum_i \sqrt{(\nabla_x \mathbf{u})_i^2+(\nabla_y \mathbf{u})_i^2} \hspace{5mm} s.t. \hspace{2mm} \mathbf{u}=\mathbf{u}_0
%\label{eq:TVL2}
%\end{equation}
%where $\mathbf{u}_0$ is usually the input image and $\mathbf{u}$ represents the restored image. It is easy to derive an $L_1$-norm counterpart of total variation from (\ref{eq:TVL2}),
%\begin{equation}
%\min_{\mathbf{u}} \|\nabla_x \mathbf{u}\|_1+\|\nabla_y \mathbf{u}\|_1 \hspace{5mm} s.t. \hspace{2mm} \mathbf{u}=\mathbf{u}_0
%\label{eq:TVL1}
%\end{equation}
 %When $p=1$, our $L_{1,1}$-regularized energy term may appear similar to (\ref{eq:TVL1}). However, there exist crucial differences between the two. First, each pairwise difference in our formulation is weighted by an affinity, which makes similar pixels even closer in the embedding space, while all components in total variation formulations are equally weighted. Second, our formulation allows direct interaction between pixels further apart by setting up connections between pixels falling into each other's neighborhood, which could be much larger than 3$\times$3, while a discretized gradient operator in total variation formulations only involves pixels within a 3$\times$3 neighborhood. These aspects of our formulation further improve the sparsity of the solution. Furthermore, the data term in total variation formulations is replaced with the orthogonality constraint in our formulation. The removal of the data term allows the embedding space to be more independent from the space of the input data. For example, the embedding space can have a different dimensionality and the embedding channels do not have to approximate the input data.

 %\noindent \textbf{Connection with 1-Laplacian}



\subsection{Numerical Solution} \label{sec:algorithm}
\noindent In the following, we first present an iterative numerical solution for a special case of the problem in (\ref{eq:PFEobjL1p}), where the $L_{1,1}$ norm is used instead of the more general $L_{1,p}$ norm.
%A new initialization scheme for this iterative solution is devised.
Then a numerical solution for the original problem in (\ref{eq:PFEobjL1p}) with the $L_{1,p}$ norm is introduced as an iteratively reweighted version of the special-case solution.

%The solution to our $L_{1,p}$-regularized objective function is devised as an iteratively reweighted version of the algorithm that solves the $L_{1,1}$-regularized objective function. Thus we will chronologically introduce the methods to solve problem (\ref{eq:PFEobjL1p}) using $L_{1,1}$ norm and $L_{1,p}$ norm, initialization and parameter selection in this subsection.

\subsubsection{Solution to ${L_{1,1}}$-regularized Objective Function}\label{sec:L11}
\noindent By setting $p=1$ in (\ref{eq:PFEobjL1p}), we obtain the ${L_{1,1}}$-regularized objective function as follows,
\begin{equation}\label{eq:PFEobjL11}
    \min_{\mathbf{Y}}{\left\|\mathbf{M}\mathbf{Y} \right\|_{1,1}} \hspace{5mm} s.t. \hspace{2mm}\mathbf{Y}^{\text T}\mathbf{DY} = \mathbf{I}.
\end{equation}
Solving this problem is challenging as it consists of $L_{1,1}$ regularization and an orthogonality constraint while most of existing numerical algorithms can only handle one of them. Here we present a numerical solution by nesting two existing solvers that handle $L_1$-regularized optimization and orthogonality constraints respectively. This solution is later accelerated with a two-stage strategy that relaxes the orthogonality constraint.

%\noindent \textbf{Enforcing Orthogonality Constraint}
Since the objective function in (\ref{eq:PFEobjL11}) is convex, we apply the Splitting Orthogonality Constraint (SOC) algorithm in \cite{lai2014splitting}. Following the derivation of the SOC algorithm, we define $\mathbf{P} = \mathbf{D}^{1/2}\mathbf{Y}$, and rewrite (\ref{eq:PFEobjL11}) as,
\begin{equation}\label{eq:PFEobjL1d1}
    \min_{\mathbf{Y}}\, \|\mathbf M \mathbf Y \|_{1,1} \hspace{3mm} s.t. \hspace{2mm}\mathbf{D}^{1/2}\mathbf{Y} = \mathbf{P}, \hspace{1mm}\mathbf{P}^{\text T}\mathbf{P} = \mathbf{I},
\end{equation}
which can be iteratively solved using Bregman iterations~\cite{bregman1967relaxation} as follows:

%\setcounter{defcounter}{0}
%\newenvironment{myequation}{%
%\addtocounter{equation}{-1}
%\refstepcounter{defcounter}
%\renewcommand\theequation{D\thedefcounter}
%\begin{equation}}
%{\end{equation}}

\begin{itemize}
  %\setlength{\itemindent}{-0.5pt}
  \setlength\itemsep{1em}
  \item[(a)]
  %$\mathbf{Y}^{(k+1)}  = \arg \underset{\mathbf{Y}} \min \;  \|\mathbf M \mathbf Y \|_{1,1} + \frac{r}{2}||\mathbf{D}^{1/2}\mathbf{Y} -\mathbf F^{(k)} ||_{2,2}^2 $,
  %in which $\mathbf F^{(k)}=\mathbf{P}^{(k)} - \mathbf{B}^{(k)}$;
  $\mathbf{Y}^{(k+1)}  = \arg \underset{\mathbf{Y}} \min \;  \|\mathbf M \mathbf Y \|_{1,1} + \frac{r}{2}||\mathbf{D}^{1/2}\mathbf{Y} - \mathbf{P}^{(k)} + \mathbf{B}^{(k)} ||_{2,2}^2 $;
  \item[(b)]
    $\mathbf{P}^{(k+1)} = \arg \underset{\mathbf{P}} \min \; \| \mathbf{P} - (\mathbf{D}^{1/2}\mathbf{Y}^{(k+1)}+\mathbf{B}^{(k)}) \|_{2,2}^2$,\\
     $ \text{s.t.} \;\; \mathbf{P}^\text{T}\mathbf{P} = \mathbf{I}$;
  \item[(c)]
  $\mathbf{B}^{(k+1)} = \mathbf{B}^{(k)} + \mathbf{D}^{1/2}\mathbf{Y}^{(k+1)} - \mathbf{P}^{(k+1)}$;
\end{itemize}
where $\mathbf{B}$ is an auxiliary matrix, and $\mathbf{B}^{(0)}=\mathbf 0$.

%\noindent \textbf{B. Solution to $\boldsymbol{L_{1,1}}$-regularized Problem}

%[[The subproblem in step (a) of the above numerical solution inherits the $L_{1,1}$-regularized energy term from (\ref{eq:PFEobjL11}). There exist many numerical solutions for optimization problems with $L_1$ regularization. For reasons discussed later, we choose to apply the Split Bregman algorithm in \cite{goldstein2009split} to solve the subproblem in step (a). The Splitting Bregman algorithm also relies on Bregman iterations. By introducing auxiliary variables, the Split Bregman algorithm solves an $L_1$-regularized optimization iteratively by transforming the original optimization into a series of differentiable unconstrained convex optimization problems. The definition of any convex optimization in the series depends on the auxiliary variables passed from the previous iteration, and convergence can be achieved within a relatively small number of iterations.]]

According to Theorem 2.1 in \cite{lai2014splitting}, the spherically constrained problem in step (b) has the following closed form solution:
\begin{eqnarray}
  \nonumber
  \mathbf{D}^{1/2}\mathbf{Y}^{(k+1)} + \mathbf{B}^{(k)} &=& \mathbf{U}\mathbf{\Sigma}_{n\times d}\mathbf{V}^{\text T}, \\
  \mathbf{P}^{(k+1)} &=& \mathbf{U} \mathbf{I}_{n\times d}\mathbf{V}^\text{T}, \label{eq:ortho}
\end{eqnarray}
where $\mathbf{U}$ and $\mathbf{V}$ are matrices with orthogonal columns from the SVD decomposition in the first step.

The subproblem in step (a) of the above numerical solution inherits the $L_{1,1}$-regularized energy term from (\ref{eq:PFEobjL11}). There exist many numerical solutions for optimization problems with $L_1$ regularization. For reasons discussed later, we choose to apply the Split Bregman algorithm in \cite{goldstein2009split} to solve the subproblem in step (a). By introducing auxiliary variables, the Split Bregman algorithm solves an $L_1$-regularized optimization iteratively by transforming the original optimization into a series of differentiable unconstrained convex optimization problems. The definition of any convex optimization in the series depends on the auxiliary variables passed from the previous iteration, and convergence can be achieved within a relatively small number of iterations. Detailed solution to the $L_{1,1}$-regularized problem in step (a) is enclosed in Appendix~\ref{appendI}.

\vspace{2mm}
\noindent \textbf{Two-Stage Implementation}
In practice, we run the following two-stage implementation to obtain a high-quality solution more efficiently.
%Due to local minimum and the highly non-convex constraint of this problem, the above algorithm does not converge effectively. In fact, the energy curve always get stuck in half way. By experiment, we found a two-stage algorithm works better. The key is to relax the orthogonality constraint in the second stage. By doing so, the energy curve can effectively diminish to almost zero.
%\vspace{2mm}

\noindent \emph{Stage I}
This stage implements the full numerical solution with nested Bregman iterations. A large penalty coefficient for the orthogonality constraint is used. The outer loop makes different dimensions of the embedded data orthogonal to each other to remove redundancy among them. This is important in avoiding naive solutions with highly redundant or even duplicate dimensions.

However, orthogonality is a highly non-convex constraint that prevents the objective function in (\ref{eq:PFEobjL11}) from settling into a truly low-energy state; and more important, it is not absolutely necessary for us to pursue an embedding whose dimensions are strictly orthogonal as long as there is not too much redundancy across different dimensions. Therefore, following a few iterations of the full numerical solution, we relax the orthogonality constraint in a second stage.

\noindent \emph{Stage II} This stage only executes the Bregman iterations in the inner loop without performing the SVD in the outer loop to strictly enforce orthogonality. Such relaxation of the orthogonality constraint allows the objective function to reach a lower energy.

Figure \ref{fig:energycurve} shows an example of the energy curve during Stage I and Stage II. It verifies our two-stage scheme can reach a lower energy than a single-stage one.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth]{energycurve.pdf}\vspace{-3mm}
  \caption{Energy curves. The black curve shows how the energy decreases with regular single-stage Bregman iterations with $\lambda = 1000, r = 100$. The dashed curves show how energy evolves with our 2-stage algorithm. The first stage is the same as the black curve. The second stage starts from iteration 50. The three dashed curves show varying convergence rates using different parameter values ($r = 100, 10, 1$ respectively for the red, blue and pink curves.)}\label{fig:energycurve}\vspace{-3mm}
\end{figure}

\vspace{1.5mm}
\noindent \textbf{Residual-Based Channel Weighting} For the sake of efficiency, we run the numerical procedure in each stage for a predefined number of iterations instead of waiting until the empirical error of every embedding channel falls below a predefined tolerance $\epsilon$.
%Besides the initialization scheme is impossible to generate equally meaningful values compared to the true global optimization solutions across dimensions and images.
Thus the obtained embedding channels differ from each other with respect to the degree of convergence. To moderate the effect of such early termination, we devise the following weighting scheme based on the residual cost of the objective function with respect to each embedding channel,
\begin{equation} \label{eq:weighting}
 \eta_{v}=\sqrt{\frac{\|\mathbf M y_{v}\|_1} { \|\mathbf D^{1/2}y_v\|_2}},\quad
\hat{y}_v=\mbox{normalize}(y_v)/\eta_{v},
\end{equation}
where $y_{v}$ and $\hat{y}_v$ are the $v$-th columns of $\mathbf Y$ obtained at the end of Stage II and the final embedding $\mathbf{\hat{Y}}$ respectively. This weighting scheme makes the importance of a channel lower if it has a larger residual cost. A comparison of PFE-based segmentations with and without residual-based channel weighting are shown in Figure \ref{fig:CMPOvsW}, where segmentation results with residual-based channel weighting are clearly better.

\begin{figure}[t]
  \centering
  %\includegraphics[width=0.6\linewidth]{images/curveplot}
 % \centering
  \includegraphics[width=\columnwidth]{CMPOvsW.pdf}\vspace{-1mm}

  %\begin{overpic}[width=1.00\columnwidth,clip,trim=20 190 40 190]{images/curveplot2}\end{overpic}
  \caption{Comparison of segmentations using piecewise flat embedding without (middle) and with (right) residual-based channel weighting. Left are input images.}\label{fig:CMPOvsW}\vspace{-2mm}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{PFEvs1LE.pdf}\vspace{-1mm}
    \caption{Comparison between PFE and 1-Laplacian~\cite{hein2010inverse}. Top row from left to right: input image; detected boundary map using~\cite{kokkinos2015pushing} for affinity matrix computation; initialization based on weighted spectral clustering as in Section~\ref{sec:ini}. Bottom row from left to right: curves of energy value $f$ (PFE) and the second smallest eigenvalue $\lambda_2$ (1-Laplacian); result of 1-Laplacian; result of PFE. 4 channels are computed in practice but only 3 embedding channels are visualized as color channels (best viewed in close-up and color image).}
    \label{fig:1laplacian}\vspace{-1mm}
\end{figure}
\vspace{1.5mm}
\noindent \textbf{Comparison to 1-Laplacian} The inverse power method in~\cite{hein2010inverse} is adopted to compute the eigenvector of 1-Laplacian with the second smallest eigenvalue. Our method enables multiple diverse embedding channels to be computed concurrently with the help of the orthogonality condition in (\ref{eq:orthog}). Comparisons of embedding results and convergence rates are shown in Figure~\ref{fig:1laplacian}. The same affinity matrix is computed from a boundary map~\cite{kokkinos2015pushing} for both methods. 1-Laplacian is applied to multiple distinct initializations independently to obtain a multi-channel embedding. The optimization processes of our method and 1-Laplacian are presented using energy value $f=\|\mathbf My\|_1$ and the second smallest eigenvalue $\lambda_2$ respectively. The convergence rates of our algorithm and 1-Laplacian are comparable. 1-Laplacian gives rise to similar embedding results across all channels despite different initializations while our method computes much more diverse channels. On average, it costs $87$s to compute one channel using 1-Laplacian and $58$s to compute 4 channels at once using our method.

\begin{figure}[t]
  \centering
  %\includegraphics[width=0.6\linewidth]{images/curveplot}
 % \centering
  \includegraphics[width=\columnwidth,clip,trim=0 145 0 0]{CMP1vsP.pdf}\vspace{.5mm}
  \includegraphics[width=\columnwidth,clip,trim=0 0 0 145]{CMP1vsP.pdf}\vspace{-1mm}
  %\begin{overpic}[width=1.00\columnwidth,clip,trim=20 190 40 190]{images/curveplot2}\end{overpic}
  \caption{Comparison of PFE-based segmentations with $L_{1,1}$ (middle) and $L_{1,0.8}$ (right) regularization. Left are input images.}\label{fig:CMP1vsP}\vspace{-2mm}
\end{figure}





\subsubsection{Solution to ${ L_{1,p}}$-regularized Objective Function}\label{sec:L1p}
\noindent To leverage algorithms for handling simpler objective functions when a more sophisticated objective function is optimized, a class of numerical methods based on iterative reweighting has been previously developed. These methods iteratively optimize a smooth or nonsmooth convex objective function dynamically weighted by coefficients evaluated from the previous iteration. For instance, IRLS\cite{daubechies2010iteratively} solves iteratively reweighted quadratic problems while IRL1~\cite{candes2008enhancing} solves iteratively reweighted $L_1$-regularized problems. Algorithms using iterative reweighting have been recently summarized in \cite{ochs2015iteratively}.
%which can be utilized to solve the problem class which sums up a convex function and a nondecreasing function applied to another convex function.
Inspired by such methods, we develop a method based on iterative reweighting to solve the $L_{1,p}$-regularized problem in (\ref{eq:PFEobjL1p}).

As done for the $L_{1,1}$-regularized problem in (\ref{eq:PFEobjL11}), the $L_{1,p}$-regularized problem in (\ref{eq:PFEobjL1p}) is also solved in two stages. The first stage of the numerical procedures for solving these two problems is completely the same. The result from the first stage initializes the second stage. In the second stage, we revise the objective function in step (a) of the procedure solving (\ref{eq:PFEobjL11}) as follows,
\begin{equation}\label{eq:PFEoptL1p}
\mathbf Y = \arg \min_{\mathbf Y} \|(\mathbf M \mathbf Y)^{\text{T}}\|_{1,p}^{p}+ \frac{r}{2}\Psi(\mathbf Y),
\end{equation}
% & = & \arg \underset{\mathbf Y} \min \sum_{k=1}^t \|\mathbf m_k^{\text{T}} \mathbf Y\|_{1}^{p-1} \|\mathbf m_k^{\text{T}} \mathbf Y\|_{1} + \Psi(\mathbf Y)
where $\Psi(\mathbf Y) = \|\mathbf D^{1/2} \mathbf Y - \mathbf P + \mathbf B \|_{2,2}^{2}$, $\mathbf P$ and $\mathbf B$ are obtained from the last outer iteration of the first stage.

We apply the majorization-minimization algorithm~\cite{ochs2015iteratively} to solve the problem in (\ref{eq:PFEoptL1p}). A Detail description is enclosed in Appendix~\ref{appendII}.

Residual-based weighting introduced earlier can still be applied to individual channels of $\mathbf Y^{(k+1)}$ obtained in the first step to improve segmentation performance. Define the result from residual-based weighting as $\mathbf{\hat{Y}}^{(k+1)}$. Then the second step of the algorithm in Appendix~\ref{appendII} is revised as follows,
\begin{equation}\label{eq:reweighting}
w_{i}^{k+1} = \mbox{max}(\alpha\|\mathbf m_i^{\text{T}} \mathbf{\hat{Y}}^{(k+1)} \|_{1},\varepsilon)^{p-1},
\end{equation}
where $\alpha$ is a constant. We experimentally found that the revised iterations can converge when $0<\alpha\le 50$. %We obtain improved segmentation results using the revised algorithm with residual-based weighting as illustrated in the next section though it is unable to prove its convergence.

A comparison of segmentations obtained through $L_{1,1}$ regularization and $L_{1,p}$ ($p=0.8$) regularization are shown in Figure \ref{fig:CMP1vsP}. $L_{1, 0.8}$ regularization gives rise to more accurate results.


\noindent \textbf{Parameter Setting} For methods developed in this paper, we select parameters as follows. In Stage I, we set the maximum number of outer iterations to 5 and the number of inner iterations to 8. In Stage II of the algorithm optimizing the $L_{1,1}$-regularized objective function in (\ref{eq:PFEobjL11}), the maximum number of iterations is set to 40. For the $L_{1,p}$-regularized objective function in (\ref{eq:PFEobjL1p}), there still exists a double loop in the second stage due to iterative reweighting. We set the maximum number of outer iterations to 5 and the number of inner iterations to 20 or less.
%has using graph-based segmentation, the regularization parameter of region size is set 200 and minimum region tolerance is set 50.
The parameter setting for $\alpha$, $\varepsilon$, $\lambda$ and $r$ will be given in the following section on image segmentation. Figure \ref{fig:embedding} shows a few embedding results. %\textcolor{red}{What is the configuration for these results?}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{embeddings1.pdf}\vspace{-1mm}
\caption{
Examples of our piecewise flat embedding. Input images are located in the first and third rows. Images in the second and fourth rows are generated by visualizing 3 embedding channels as color channels. Note that the embedding results clearly exhibit piecewise flatness.}
\label{fig:embedding}\vspace{0mm}
\end{figure}

